Human Activity Recognition in an Open World

Managing novelty in perception-based human activity recognition (HAR) is critical in realistic settings to improve task performance over time and ensure solution generalization outside of prior seen samples. Novelty manifests in HAR as unseen samples, activities, objects, environments, and sensor changes, among other ways. Novelty may be task-relevant, such as a new class or new features, or task-irrelevant resulting in nuisance novelty, such as never before seen noise, blur, or distorted video recordings. To perform HAR optimally, algorithmic solutions must be tolerant to nuisance novelty, and learn over time in the face of novelty. This paper 1) formalizes the definition of novelty in HAR building upon the prior definition of novelty in classification tasks, 2) proposes an incremental open world learning (OWL) protocol and applies it to the Kinetics datasets to generate a new benchmark KOWL-718, 3) analyzes the performance of current state-of-the-art HAR models when novelty is introduced over time, 4) provides a containerized and packaged pipeline for reproducing the OWL protocol and for modifying for any future updates to Kinetics. The experimental analysis includes an ablation study of how the different models perform under various conditions as annotated by Kinetics-AVA. The protocol as an algorithm for reproducing experiments using the KOWL-718 benchmark will be publicly released with code and containers at https://github.com/prijatelj/human-activity-recognition-in-an-open-world. The code may be used to analyze different annotations and subsets of the Kinetics datasets in an incremental open world fashion, as well as be extended as further updates to Kinetics are released.

==> graphics/tables/timetable.tex <==
%% The table of notation and definitions
%\begin{table*}
%\scalebox{0.82}{
%{\setlength{\tabcolsep}{0.41em}
\newpage
\onecolumn
{
\rowcolors{1}{white}{lightgray}
%\small
%\centering
    \begin{longtable}{p{0.13\textwidth}p{0.66\textwidth}p{0.12\textwidth}}
        \caption{
            \label{tab:timetable}
            The initial timetable of tasks given previous prioritization as of 2021-09-30.
            %Further task and sub-task details \TODO{in GitLab Issues with associated deadlines if adjustments are needed. Though this takes time to manage}.
            ``\textit{Macro}'' stands for the main objectives to be done during the week.
            The rest of the rows in the week are the individual tasks, probably still missing sub-tasks given space.
            Note that the listed tasks per week are not necessarily 1-to-1 in time commitment/effort.
            As the paper is written, placeholders and content will be added to the supplementary material.
            The linked numbers are the numbered TODOs in this overview that relate to each task item.
        } \\
    \label{tab:timetable}
        \textbf{Week \& Todos} & \textbf{Task List} & \textbf{Assigned To} \\
        \hline
        \endfirsthead
        \textbf{Week \& Todos} & \textbf{Task List} & \textbf{Assigned To} \\
        \hline
        \endhead
    %% Probability Notation
         Sept. 26--Oct. 2
            & \textit{Macro: Plan made, Paper Draft w/o Results}
            & 
            \\
            \ref{todo:litrev_check}
            & Finish Lit. Review: Check to ensure our space of novel contrib is secure.
            & Derek
            \\
            & Finish overview \& share overleaf.
            & Derek
            \\
            \ref{todo:inc_owl_vis} 
            & Begin 1st Draft main paper non-results content.
            & Derek
            \\ \ref{todo:rmk4ink7}, \ref{todo:code_class_map}, \ref{todo:data_detail}, \ref{todo:find_novel_set_k7}
            &  Begin: Obtain code automation of Mapping Kinetics-400 $\rightarrow$ K-700 $\rightarrow$ PAR
            &  Sam
            \\
            &  Begin: Dataloaders for Kinetics 400, K-700, and PAR (same data format for agent models)
            & Sam
            \\
            \ref{todo:augs}, \ref{todo:auto_aug} 
            &  Begin: PyTorch visual augmentation  as part of loading pipeline and implement saving augs (Frames or whole videos) with random seed set (0 or otherwise)
            & Sam
            \\
         %\rowcolor{lightgray} 
        \hline
        Oct. 3--9
            & \textit{Macro: Data splits \& Loaders Done, X3D on 1st increment data, EVM and Clustering post-X3D, Eval Code
            }
            & 
            \\
            \ref{todo:inc_owl_vis} 
            & Finish 1st Draft main paper non-results content.
            & Derek
            \\
            & Feedback and Revise 1st Draft w/o Results main text
            & Walter \& Sam then Derek
            \\
            \ref{todo:data_detail}, \ref{todo:find_novel_set_k7}, \ref{todo:auto_owl}, \ref{todo:auto_owl_factors}
            &  Data split and loader process for incremental OWL with a random seed (0).
            & Derek
            \\
            \ref{todo:rmk4ink7}, \ref{todo:code_class_map},
            \ref{todo:data_detail}, \ref{todo:find_novel_set_k7}, \ref{todo:auto_owl}, \ref{todo:auto_owl_factors}
            & \textbf{Dev. \& Debug Time} for ensuring the data splitting, loading, and details are finalized. This is critical to get finished for the rest of the project.
            & Sam \& Derek
            \\
            \ref{todo:augs}, \ref{todo:auto_aug} 
            &  Continue: PyTorch visual augmentation  as part of loading pipeline and implement saving augs (Frames or whole videos) with random seed set (0 or otherwise)
            & Sam
            \\
            & Begin: Figure out clustering, and update processes, Initial code for this
            & Derek
            \\
        \hline
        Oct. 10--16
            & \textit{Macro: Debug \& Training Time Buffer, X3D Exp 2 \& 3 w/o feedback}
            & 
            \\
            & Feedback from Non-ND authors \& Revise 2nd Draft w/o Results main text
            & Other Authors \& then Derek
            \\
            \ref{todo:k4plm_vs_finetune}
            & Finish X3D on first increment with Frozen weights and multi-objective case.
            & Sam
            \\
            \ref{todo:auto_owl}
            & Implement EVM generic pipeline (train, eval, save/load) and Clustering no-feedback update
            & Derek
            \\
            \ref{todo:errbar}
            & Code Evaluation measure functions/pipeline, code for visuals
            & Derek
            \\
            & Implement Transformer Model: Timesformer, ViVet, CLIP/ActionCLIP or other 
            & Derek
            \\
        \hline
        Oct. 17--23
            & \textit{Macro: Debug \& Training Time Buffer, Finish MVP with results, Begin MVP++}
            & 
            \\
            & Targeted Feedback \& Revise 3rd Draft main text \textbf{w/ MVP Results}. 
            & Walter \& Sam then Derek
            \\
            &  Debug the implemented transformer and get running on all data.
            &  Derek
            \\
        \hline
        Oct. 24--30
            & \textit{Macro: Finalize DARPA Eval agent and code for Nov. 1st.}
            & 
            \\
            & 
            &  
            \\
            & 
            &  
            \\
        \hline
        Oct. 31--Nov. 6
            & \textit{Macro: }
            & 
            \\
            & Send Draft out for External Feedback \& Revise N-th Draft \textbf{w/ Results}. 
            & Walter, Derek, others
            \\
            & 
            &  
            \\
            & 
            &  
            \\
        \hline
        \hline
            \centering\textbf{CVPR DL}
            &  \centering\textbf{ Be done with experiments for CVPR SUBMISSION DEADLINE! MVP++}
            &  
            \\
        \hline
        \hline
        Nov. 7--13
            & \textit{Macro: Final DARPA Eval submission Nov. 16th}
            & 
            \\
            & Revise N-th Draft based on External Feedback.
            & Walter then Derek
            \\
            & 
            &  
            \\
            & 
            &  
            \\
        \hline
        Nov. 14--20
            & \textit{Macro: Final submission for CVPR and DARPA Eval Nov. 16th}
            & 
            \\
            & Polish N-th Draft. Ensure CMT is updated w/ latest before Tuesday.
            & All Authors
            \\
            & 
            &  
            \\
        \hline
        Nov. 21--23  
            & \textit{Macro: Finish any loose ends and finalize \& submit the Supp Mat.}
            & 
            \\
            & Refine and Submit the Supplementary Material.
            & Derek \& Everyone
            \\
            & Submit to Arxiv \& Publicly Announce (Marketing).
            &  
            \\
    \end{longtable}
}
\newpage
\twocolumn
%}}
%\end{table*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> writing/5.2.1_vtransforms_timeseries.tex <==
\begin{figure*}[t]
    \centering
    \small
    
    \textbf{\cc{Tolerance to Visual Transforms for HAR Classification Non-Cumulative Performance on KOWL-718}}
    
    \textbf{Training Set}
    \hfill
    \textbf{Testing Set}
    
    \includegraphics[width=\linewidth]{graphics/exp2/wide/non-cumu/task-perf/train_acc.pdf}
    \includegraphics[width=\linewidth]{graphics/exp2/wide/non-cumu/task-perf/train_mcc.pdf}
    \includegraphics[width=\linewidth]{graphics/exp2/wide/non-cumu/task-perf/train_nmi.pdf}
    \caption{
        \small
        The novelty detection and recognition performance of the predictors over incremental learning on the Kinetics Unified dataset.
        Both novelty detection and recognition are assessed at the beginning during \textbf{pre-feedback} of every increment, and the results are on the combination of \textbf{all new data} in that increment.
    }
    \label{fig:exp2:task}
\end{figure*}

\begin{figure*}[t]
    \centering
    \small
    
    \textbf{\cc{Placeholder for} Tolerance to Nuisance Novelty for Novelty Detection and Recognition Non-Cumulative Performance on KOWL-718}
    
    \textbf{Novelty Detection}
    \hfill
    \textbf{Novelty Recognition}
    
    \includegraphics[width=\linewidth]{graphics/exp2/wide/non-cumu/task-perf/train_acc.pdf}
    \includegraphics[width=\linewidth]{graphics/exp2/wide/non-cumu/task-perf/train_mcc.pdf}
    \includegraphics[width=\linewidth]{graphics/exp2/wide/non-cumu/task-perf/train_nmi.pdf}
    \caption{
        \small
        The novelty detection and recognition performance of the predictors over incremental learning on the Kinetics Unified dataset.
        Both novelty detection and recognition are assessed at the beginning during \textbf{pre-feedback} of every increment, and the results are on the combination of \textbf{all new data} in that increment.
    }
    \label{fig:exp2:task}
\end{figure*}


\cc{Time-series non-cumulative or cumulative performance per predictor given each visual transform.}
The difference in classification performance on just Kinetics-400 motivated the analysis of predictor tolerance to nuisance novelty on KOWL-718.
To perform this analysis, the saved checkpoints after post-feedback of every predictor evaluated on KOWL-718 were loaded and then the evaluation process continued but using the visually transformed video samples instead of the originals.
Each visual transform was assessed in separate runs from each other.
The incremental learning process only proceeded from the current increment's post-feedback evaluation to the pre-feedback evaluation on the next increment's new data.
This means that the incremental learning from beginning to end on only those visual transforms was not assessed, and allowed us to treat the visual transforms as nuisance novelty for the predictor at both the post-feedback and pre-feedback evaluation for the finetuned ANNs given that they did not update their state using those samples.
The GMM FINCH predictors update their state with or without feedback and as such, the visual transforms were used in updating the internal state of the predictor for both the current increment's post-feedback videos and next increment's pre-feedback videos.
Still, even for the 100\% feedback predictors, no activity class feedback was given for the visually transformed samples.
